Large Language Models as Superpositions of Cultural Perspectives

Large Language Models (LLMs) are often misleadingly recognized as having a personality or a set of values. We argue that an LLM can be seen as a superposition of perspectives with different values and personality traits. LLMs exhibit context-dependent values and personality traits that change based on the induced perspective (as opposed to humans, who tend to have more coherent values and personality traits across contexts). We introduce the concept of perspective controllability, which refers to a model's affordance to adopt various perspectives with differing values and personality traits. In our experiments, we use questionnaires from psychology (PVQ, VSM, IPIP) to study how exhibited values and personality traits change based on different perspectives. Through qualitative experiments, we show that LLMs express different values when those are (implicitly or explicitly) implied in the prompt, and that LLMs express different values even when those are not obviously implied (demonstrating their context-dependent nature). We then conduct quantitative experiments to study the controllability of different models (GPT-4, GPT-3.5, OpenAssistant, StableVicuna, StableLM), the effectiveness of various methods for inducing perspectives, and the smoothness of the models' drivability. We conclude by examining the broader implications of our work and outline a variety of associated scientific questions. The project website is available at https://sites.google.com/view/llm-superpositions .

==> backup_markdown_tables.tex <==

% Mean value change

% |                  | Conformity   | Tradition     | Benevolence  | Universalism | Self-Direction | Stimulation  | Hedonism     | Achievement  | Power        | Security     |
% |------------------|--------------|---------------|--------------|--------------|----------------|--------------|--------------|--------------|--------------|--------------|
% | 10/12 - 12/14 yo | 0.05         | -0.09         | 0.02         | 0.04         | 0.30           | 0.22         | 0.29         | 0.17         | 0.16         | 0.01         |
% | 20 - 28 yo       | 0.53         | 0.04          | 0.23         | 0.40         | 0.17           | -0.20        | -0.06        | -0.23        | 0.20         | 0.22         |
% | priming (ben)    | -            | -             | 0.53         |              |                |              |              |              |              |              |
% | priming (control)| -            | -             | -0.42        |              |                |              |              |              |              |              |
% |------------------|--------------|---------------|--------------|--------------|----------------|--------------|--------------|--------------|--------------|--------------|
% | chess - grammar  | -2.98156274  | -0.69726061   | 0.83396232   | 1.08905467   | 0.32078088     | 2.03119844   | 0.96185520   | -0.50195675  | -0.47096640  | -2.44182449  |
% | chess - history  | -2.92898921  | -0.76091065   | 1.88820452   | 1.55551103   | 2.00366513     | 1.58134478   | -0.43472147  | -2.22123414  | -1.50068110  | -0.56834461  |
% | chess - joke     | -2.06504286  | -1.25988912   | 2.08184620   | 3.59401403   | 2.40735164     | 0.83328996   | -0.49762484  | -3.03743693  | -2.55671150  | -0.84699873  |
% | chess - poem     | -1.83969459  | -1.77651364   | -0.96058745  | -0.84129671  | -0.67877592    | 2.15411118   | 1.39240277   | 0.33714691   | -0.30440379  | -0.80606303  |
% | chess - religion | -2.21179327  | -1.41274437   | 1.93146654   | 2.90042037   | 3.17956839     | 0.50391657   | -0.70720607  | -3.26462314  | -1.76504458  | -1.02982999  |
% | chess - tax      | -2.51031173  | -0.85317756   | 1.65958777   | 2.99923552   | 2.36940951     | 0.91918219   | -0.29944552  | -2.61169434  | -1.27442224  | -1.53796396  |
% | chess - vacation | -2.21479763  | -1.58481235   | 2.62401683   | 2.34287110   | 3.25340999     | 0.55309436   | -0.01213460  | -3.18688350  | -3.65225239  | -0.39975822  |
% | grammar - history| -0.06904032  | -0.06254326   | 0.97210756   | 1.51533814   | 1.51533814     | -0.45831013  | -1.62581546  | -1.57059257  | -0.90133242  | 1.51247257   |
% | grammar - joke   | 0.52765105   | -0.39018078   | 1.34045498   | 1.95186122   | 1.95186122     | -1.13618992  | -1.63441416  | -2.41777157  | -1.76874034  | 1.44897392   |
% | grammar - poem   | 1.76423022   | -0.76051822   | -1.55400610  | -1.83877484  | -0.91155626    | 0.18983143   | 0.46934298   | 0.80516216   | 0.26603137   | 1.57821681   |
% | grammar - religion| 0.49377653  | -0.61941530   | 1.18113715   | 1.87254559   | 2.65964100     | -1.51311671  | -1.79478669  | -2.44780196  | -1.25956624  | 1.50883063   |
% | grammar - tax    | 0.40506036   | -0.26665413   | 0.88714800   | 1.89998629   | 1.88376224     | -0.89046486  | -1.40853198  | -1.94630201  | -0.84533431  | 0.78000347   |
% | grammar - vacation| 0.51707951  | -0.81057596   | 1.84013109   | 1.37951394   | 2.65410840     | -1.32754647  | -1.12701942  | -2.51583159  | -2.74029302  | 1.64177284   |
% | history - joke   | 0.57112160   | -0.31691516   | 0.50725782   | 1.27997700   | 1.27997700     | -0.69827654  | -0.09119534  | -0.98644334  | -0.80884568  | -0.17919931  |
% | history - poem   | 1.74173804   | -0.67903183   | -2.52945455  | -2.13101825  | -2.13101825    | 0.63187519   | 2.17230524   | 2.56105778   | 1.34520617   | -0.11728865  |
% | history - religion| 0.53948348  | -0.55105660   | 0.33468272   | 0.99488080   | 0.99488080     | -1.06485255  | -0.35005703  | -0.75816291  | -0.47939755  | -0.25752162  |
% | history - tax    | 0.45630149   | -0.21252532   | 0.01101598   | 0.43734355   | 0.43734355     | -0.49083441  | 0.13683395   | -0.39930268  | -0.10886605  | -0.77096870  |
% | history - vacation| 0.55897989  | -0.53333079   | 1.12750617   | 0.99323509   | 0.59276076     | -0.91205642  | 0.48834169   | -1.02017380  | -1.77156127  | 0.13740821   |
% | joke - poem      | 0.84073179   | -0.40732067   | -2.59553456  | -4.32968592  | -4.32968592    | 1.28232181   | 2.14682775   | 3.34168902   | 2.43935769   | 0.07431940   |
% | joke - religion  | -0.05094724  | -0.29517705   | -0.16197256  | -0.21068457  | -0.21068457    | -0.33791562  | -0.25394310  | 0.35040553   | 0.20192810   | -0.07125671  |
% | joke - tax       | -0.16575221  | 0.02977362    | -0.46376065  | -0.28439597  | -0.28439597    | 0.14513111   | 0.21768319   | 0.60773770   | 0.55049708   | -0.64508186  |
% | joke - vacation  | -0.03508289  | -0.51939012   | 0.43402611   | -0.64138546  | -0.64138546    | -0.23917128  | 0.55463724   | 0.00530648   | -1.00962849  | 0.32463722   |
% | poem - religion  | -0.95744210  | 0.04280859    | 2.46148222   | 3.52501256   | 3.52501256     | -1.65054619  | -2.27319185  | -3.67280114  | -1.63839226  | -0.15656722  |
% | poem - tax       | -1.21810336  | 0.30818218    | 2.22643002   | 3.66538272   | 3.66538272     | -1.03293194  | -1.91229282  | -2.94988675  | -1.14216538  | -0.74204848  |
% | poem - vacation  | -0.94876129  | -0.21041299   | 3.12757924   | 2.94422713   | 2.94422713     | -1.46297522  | -1.64590854  | -3.51565994  | -3.57614014  | 0.26815060   |
% | religion - tax   | -0.11649450  | 0.24884170    | -0.30161027  | -0.05825151  | -0.05825151    | 0.45987650   | 0.45921344   | 0.32105528   | 0.31512753   | -0.63249419  |
% | religion - vacation| 0.01688477 | -0.21818688   | 0.60250742   | -0.40005107  | -0.40005107    | 0.07959032   | 0.78310491   | -0.35955436  | -1.04423919  | 0.41268959   |
% | tax - vacation   | 0.13562852   | -0.42409599   | 0.91826922   | -0.35765146  | -0.35765146    | -0.36256687  | 0.32855686   | -0.62542779  | -1.35244271  | 0.90731786   |
% |------------------|--------------|---------------|--------------|--------------|----------------|--------------|--------------|--------------|--------------|--------------|
% | chat - code_cpp  | -1.04751391  | -1.05371770   | 4.00016234   | 3.58232118   | 5.30729566     | -1.25595165  | -0.69224702  | -2.32188880  | -5.85922283  | 1.80991958   |
% | chat - code_py   | 1.21473688   | -0.57309555   | 3.08544386   | 2.50496392   | 3.92933596     | -1.55949331  | -1.17105672  | -1.83247762  | -3.31650248  | 2.00464068   |
% | chat - conf_toml | -0.24656235  | -0.48906525   | 0.87491052   | 0.45240155   | 1.72526483     | -0.60277116  | -1.18359011  | -0.34808370  | 0.27375294   | 0.37620039   |
% | chat - latex     | 0.66593453   | -0.19983377   | 1.36201039   | 0.97342761   | 1.80820315     | -1.33484009  | -1.30822070  | -0.28186573  | -1.40209107  | 1.65871566   |
% | code_cpp - code_py | 1.96810066 | 0.49338975    | -0.93010486  | -0.80849775  | -1.36872942    | -0.65478270  | -0.52188859  | 0.18341822   | 0.20002444   | 0.57860779   |
% | code_cpp - conf_toml | 0.72527207 | 0.56122992   | -3.64881876  | -2.94317397  | -3.34287759    | 0.48424871   | -0.65917273  | 1.72717360   | 5.01837865   | -1.15930250  |
% | code_cpp - latex | 1.34847888   | 0.71731525    | -1.92834522  | -2.14679809  | -2.22120534    | -0.53494609  | -0.77523607  | 1.54474206   | 1.48112068   | 0.55585199   |
% | code_py - conf_toml | -1.27461011 | 0.07743115   | -2.55135650  | -1.97116214  | -2.04313420    | 0.88035912   | -0.23724540  | 1.36630789   | 3.24935989   | -1.45865850  |
% | code_py - latex  | -0.17822056  | 0.30424142    | -1.22909600  | -1.31256769  | -1.23023529    | -0.07233364  | -0.34072219  | 1.25953626   | 1.09582580   | 0.12624635   |
% | conf_toml - latex | 0.78697984  | 0.23417070    | 0.70331665   | 0.53107672   | 0.38344019     | -0.78024872  | -0.08408961  | 0.02932610   | -1.50173201  | 1.27814555   |
% |--------------------------|--------------|-------------|--------------|--------------|----------------|---------------|--------------|--------------|--------------|--------------|
% | classical - gospel       | -0.12318375  | -1.14187246 | -0.44523927  | 0.39916517   | 1.04021807     | 1.66824563    | -0.63109361  | 0.36752686   | 0.13640451   | -1.28883747  |
% | classical - heavy metal  | 1.55869967   | 1.61281147  | 0.44901054   | -0.18212056  | 0.49727859     | -0.05710372   | -1.96068414  | -0.84176496  | 0.14436996   | -0.47231744  |
% | classical - hip-hop      | 0.96345702   | 0.68423967  | 0.37219595   | 0.35397492   | 0.99997998     | 0.08356408    | -1.45651215  | -0.32388251  | -0.20089638  | -1.10795919  |
% | classical - jazz         | 1.06067671   | 1.24140652  | 0.10018849   | 0.52106491   | -0.14953134    | 0.04422417    | -2.32009343  | 0.11600721   | 0.45468666   | 0.41894099   |
% | classical - reggae       | 0.84320096   | 0.16336305  | -0.05124397  | -0.65593821  | 0.52345603     | 1.17710090    | -1.87703758  | 0.90684968   | -0.01801081  | -0.57960844  |
% | gospel - heavy metal     | 1.58313646   | 2.89137378  | 0.93903711   | -0.57476050  | -0.61261844    | -1.97329976   | -1.14025403  | -1.15489825  | 0.01585955   | 0.77536942   |
% | gospel - hip-hop         | 1.02174363   | 1.72972302  | 0.86957238   | -0.05750729  | -0.09482795    | -2.20405380   | -0.62490809  | -0.69692206  | -0.31470240  | 0.39882026   |
% | gospel - jazz            | 1.11403297   | 2.64543970  | 0.58070196   | 0.12557489   | -1.18450962    | -2.05664160   | -1.57961899  | -0.26499714  | 0.30413923   | 1.69739631   |
% | gospel - reggae          | 0.90990353   | 1.43007170  | 0.43166385   | -1.04962132  | -0.53056908    | -0.46925529   | -1.11851147  | 0.47001562   | -0.15696700  | 0.83750079   |
% | heavy metal - hip-hop    | -0.70209759  | -0.73481489 | -0.09073040  | 0.53511866   | 0.54746163     | 0.17392416    | 0.95860749   | 0.60911524   | -0.31345748  | -0.51630905  |
% | heavy metal - jazz       | -0.45265400  | -0.55629646 | -0.37473078  | 0.69318300   | -0.65406040    | 0.12118198    | -0.81675006  | 0.97787304   | 0.27110593   | 0.87498473   |
% | heavy metal - reggae     | -0.82836952  | -1.60141036 | -0.54488854  | -0.46659309  | 0.05502615     | 1.38481178    | -0.09693715  | 1.80015626   | -0.16353932  | -0.04263898  |
% | hip-hop - jazz           | 0.20229576   | 0.32772917  | -0.29124368  | 0.18650984   | -1.15186110    | -0.04907299   | -1.56189438  | 0.45975194   | 0.59986235   | 1.58138141   |
% | hip-hop - reggae         | -0.13372009  | -0.58862044 | -0.46381098  | -1.02255767  | -0.46273625    | 1.45582257    | -0.86774350  | 1.33699375   | 0.18961973   | 0.56389034   |
% | jazz - reggae            | -0.32291686  | -1.20228239 | -0.16480122  | -1.16455795  | 0.67226135     | 1.39146381    | 0.63615287   | 0.80335685   | -0.48323280  | -1.03239764  |






==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

